Exploiting Fine-Grain Ordered Parallelism in Dense Matrix Algorithms

Dense linear algebra kernels are critical for wireless applications, and the oncoming proliferation of 5G only amplifies their importance. Many such matrix algorithms are inductive, and exhibit ample amounts of fine-grain ordered parallelism -- when multiple computations flow with fine-grain producer/consumer dependences, and where the iteration domain is not easily tileable. Synchronization overheads make multi-core parallelism ineffective and the non-tileable iterations make the vector-VLIW approach less effective, especially for the typically modest-sized matrices. Because CPUs and DSPs lose order-of-magnitude performance/hardware utilization, costly and inflexible ASICs are often employed in signal processing pipelines. A programmable accelerator with similar performance/power/area would be highly desirable. We find that fine-grain ordered parallelism can be exploited by supporting: 1. fine-grain stream-based communication/synchronization; 2. inductive data-reuse and memory access patterns; 3. implicit vector-masking for partial vectors; 4. hardware specialization of dataflow criticality. In this work, we propose, REVEL, as a next-generation DSP architecture. It supports the above features in its ISA and microarchitecture, and further uses a novel vector-stream control paradigm to reduce control overheads. Across a suite of linear algebra kernels, REVEL outperforms equally provisioned DSPs by 4.6x-37x in latency and achieves a performance per mm 2 of 8.3x. It is only 2.2x higher power to achieve the same performance as ideal ASICs, at about 55% of the combined area.

==> challenges.tex <==
\section{DSP Workload Challenges and Insights} \label{sec:challenges}

In this section we characterize the two main challenges for DSP algorithms,
which relate to the problem of control and parallelism.  Overall,
we discover five necessary architecture features, and the next
section discusses their implementation.

\subsection{Inductive Control and Memory} \label{sec:access}

One of the primary reasons for ineffective vectorization in DSP 
algorithms is the control overhead
in specifying the data access pattern and its relationship with computation
over different phases of the algorithm.  This comes from both the small
matrix rows being indivisible by vector length,  control instructions which
modulate the vector length, as well as any difficult-to-vectorize
outer loop code.

%\footnote{We are 
%careful to note that there are other reasons why \emph{streams} 
%are used in other ISA besides just control overhead, for example to encode
%alias freedom.} 

An alternative technique to hiding control overheads is to use coarse grain
patterns of memory access, called
\emph{streams}~\cite{imagine,rsvp,stream-dataflow}.  Broadly, a \emph{stream}
in this paper is a predefined access pattern with a few parameters; a stream
does not imply strictly contiguous access.  The promise of using streams here
is that a small number of parameters could perhaps specify a complex pattern of
array accesses, thereby reducing the control overhead.  Using streams for DSP
workloads is quite plausible given that the types of memory access is not
overly broad.  

The question then becomes \emph{what type of stream patterns should 
hardware employ?}  The tradeoff of a more complex pattern is
less control overhead at the cost of 1. complexity in the ISA, 
burdening the compiler or programmer, and 2. complexity in hardware,
in generating more complex addresses.  

\paragraph{Access Pattern Definition}
To analyze this problem quantitatively, we formulate a definition of a set 
of access patterns that are useful in the domain of dense linear algebra. 
First, an access pattern has a dimension $d$, and a corresponding number of
iterators $i$, $j$, $k$, and so on.
which are the basis of the iteration domain.  An array access
function maps elements in the iteration domain to addresses 
through an affine function specified
by a multiplier for each iterator $c_i$, $c_j$, $c_k$.  For example
in dimension 3, this would be $k * c_k +  j * c_j + i * c_i$.  The access
pattern also has an initial length $n_i$, $n_j$, $n_k$ for each dimension (ie.
number of iterations).

\begin{figure}
\begin{minipage}{0.59\linewidth}
\footnotesize
\begin{lstlisting}[mathescape=true]
for k=0 to $n_k$
  for j=0 to $n_j$
    for i=0 to $n_i$
      a[$k * c_k +  j * c_j + i * c_i$] 
\end{lstlisting}
\end{minipage}
\begin{minipage}[r]{0.38\linewidth}
\includegraphics[width=\linewidth]{figs/acc-rect.pdf}
\end{minipage}
  \captionof{lstlisting}{3D Rectangular Access Pattern (RRR) }
  \label{fig:rii}
\vspace{0.2in}
\begin{minipage}[c]{0.59\linewidth}
\footnotesize
\begin{lstlisting}[mathescape=true]
for k=0 to $n_k$
  for j=0 to $n_j + k * s_{kj}$
    for i=0 to $n_i + k * s_{ki}  + j*s_{ji}$
      array[$k * c_k +  j * c_j + i * c_i$] 
\end{lstlisting}
\end{minipage}
\begin{minipage}[r]{0.38\linewidth}
\includegraphics[width=\linewidth]{figs/acc-ind.pdf}
\end{minipage}
  \captionof{lstlisting}{3D Inductive Access Pattern (RII)}
  \label{fig:rrr}
\end{figure}
%    ... = array[$i * c_i +  j$] 



\emph{Inductive} access patterns, are those that modify their length
as a function of prior iterators, which can be specified through
a set of ``stretch'' parameters $s_{ij}$.  Here, $s_{ij}$
represents the change in length $n_j$
caused by the value of iterator $i$.  For example, in dimension 3, an
inductive access length can be captured by $n_i + k * s_{ki}  + j * s_{ji}$.
Figures~\ref{fig:rrr} and~\ref{fig:rii} show a non-inductive (henceforth
\emph{rectangular}) and inductive access pattern respectively, with
a visual depiction of a possible pattern.

We ease the presentation in comparing inductive and non-inductive access 
capability through a simple notation.  For a given access capability, 
an R denotes a rectangular dimension, and I denotes inductive dimension; 
RI would be a 2-dimensional capability with induction in second 
dimension.
%\footnote{Note that an inductive first dimension
%is meaningless as there are no prior loop iterators to  be inductive with
%respect to.}.  


\begin{figure} [t]
\begin{center}
\includegraphics[width=\linewidth]{figs/acc-len-small.pdf}
\end{center}
  \caption{Access Lengths of various Capabilities}
\label{fig:acc-len}
\end{figure}

\begin{figure} [t]
\begin{center}
\includegraphics[width=\linewidth]{figs/acc-iters-small.pdf}
\end{center}
  \caption{Control overhead of various Capabilities.  White bars indicate
  control overhead if stream-reuse technique is enabled.}
\label{fig:acc-iters}
\end{figure}


\begin{figure}[t]
\begin{minipage}{0.42\linewidth}
\footnotesize
\begin{lstlisting}[mathescape=true]
  for j=0 to $n_j$
    for i=0 to $n_i$
      a[$j * c_j$] 
\end{lstlisting}
\end{minipage}
$\,\to\,$
\begin{minipage}{0.42\linewidth}
\footnotesize
\begin{lstlisting}[mathescape=true]
  for j=0 to $n_j$
    temp = a[$j * c_j$] 
    for i=0 to $n_i$
\end{lstlisting}
\end{minipage}
  \captionof{lstlisting}{Example of Stream Reuse Pattern}
  \label{fig:rr-reuse}
\end{figure}

To analyze the ``power'' of an access capability, we require an algorithm
to determine the $c$, $n$, and $f$ parameters for each memory accesses.
To do this, we iterate over the loop nest for each access, from inner-most
to outer-most, and attempt to map the stride of the address and loop termination
condition to the $c$ and $n,f$ parameters respectively.  In the common case,
each loop dimension maps to a dimension of the address capability, but sometimes
 a single capability dimension can map all loop nest levels (eg. a[$k$][$j$][$i$]
where all $n$ are equal to array dimension).

We implement the following analysis in an LLVM~\cite{llvm} static pass, and rely
on scalar evolution analysis~\cite{scev} for the closed-form representation 
of address patterns and loop termination with respect to induction variables.
The ``access length'' is the number of iterations of the loop which the pattern
describes, shown in Figure~\ref{fig:acc-len}. 
We also calculate the number of effective memory instructions
per inner-loop iteration, ``Mem. Insts/Iter'', which is a measure of the control
overhead (Figure~\ref{fig:acc-iters}).


\paragraph{Access Length Analysis}  Regular workloads like GEMM require only a
low dimension rectangular access pattern for a long length.  However, the same
Cholesky, QR, and SVD show much higher lengths \emph{only} with inductive 
access capability.  This benefit translates to fewer memory instructions
per-iteration.  A value of less than 1 in Figure~\ref{fig:acc-iters} means that
fewer than one control instructions would need to be issued per cycle.  This
helps to explain \emph{why} vector instructions alone are insufficient for
parallelism -- because they require too much specification of work.
Fortunately, the RI capability always either achieves a control
overhead below 1 inst/iter, or matches the-higher dimension capability, leading
to the first feature:

\textbf{Feature 1: The accelerator can nearly eliminate control overhead
by using a RI-based access-capability model (2D induction-based) in its
hardware/software interface.}



\paragraph{Stream-reuse}  A second consideration is for addresses which repeat 
during the inner iteration, as shown in Figure~\ref{fig:rr-reuse}. Simply setting 
$c_i$ of the innermost dimension to 0 is correct, but implies a re-accesses of 
the same memory
multiple times and also wastes a dimension of the access capability.

If the hardware-software interface can indicate a ``stream-reuse'' pattern --
the length $n_r$ and stretch $s_r$ specifically for stream reuse, 
then not only is a dimension of the access pattern spared,
it becomes easier for the hardware to exploit reuse of these variables locally.  
The control overhead benefits are
modest (shown in Figure~\ref{fig:acc-iters} as white lines on bars), but can often
reduce memory bandwidth requirement.

\textbf{Feature 2: The interface to data access
should expose stream-reuse patterns to the hardware.}

\subsection{Parallelizing with Fine-grain Dependences}

The other primary opportunity to improve performance of dense linear algebra
codes is to parallelize across code-regions. Often, and particularly for
matrix factorization, there are several computation regions that exhibit
concurrency, but have fine-grain dependences within their respective iteration
domains.  These dependences make parallelization difficult.

We show examples of these dependences in two example workloads, QR 
and Cholesky decomposition,
in Figures~\ref{fig:qr-dep} and~\ref{fig:chol-dep}.  Each figure shows a 
depiction of the computationally important code regions (corresponding to loop
nests), separated by horizontal lines; note that an outer \texttt{for k}
loop encloses both examples.  A dataflow graph representation 
of each region appears to the right.  Yellow rectangles represent memory
access streams, and red rounded shapes indicate computation.  Edges represent
data dependences. Black edges have a uniform production to consumption rate,
while gray edges are non-uniform, and they are labeled with their 
production:consumption rate.  A higher production (on the left) 
indicates \emph{multiple-reuse}, while 
higher consumption (on the right) indicates a \emph{reduced-use}.  

\begin{figure}[t]
\includegraphics[scale=0.5]{./figs/householder.pdf}
\caption{Computing kernels of QR (\%'s: ideal execution rate).}
\label{fig:qr-dep}
\end{figure}


\paragraph{QR} Here we show the calculation of the R matrix using
householder reflections~\cite{intro_num_anal}.  The first three regions 
compute the householder vector, and the second two compute the householder
rotation.  As alluded to in section~\ref{sec:access}, the vectorization opportunity
within each region is limited due to the small lengths.  However, there is
ample parallelism across regions.  For example, across the outer \texttt{for k}
loop, it is possible to execute the first three regions in pipeline
parallel fashion, where ``Norm Computation'' is working on iteration \texttt{k},
''Divisor Calculation'' is working on iteration \texttt{k-1} and
``Normalization'' is working on iteration \texttt{k-2}.  The
reduced-use dependence before the divisor calculation and multiple-reuse of the
generated value afterwards, make this difficult to parallelize
unless expressed directly.

The final two regions also 
exhibits a common non-uniform production to consumption pattern.  Here, the
matrix-vector multiply produces a vector, v, reused multiple times by
an outer-product-subtraction region.  
%Note that there is ample parallelism
%here even within the same \texttt{for i} iteration.

\textbf{Feature 3: The hardware/software interface must expose a mechanism
to support fine grain dependences with multiple-reuse and reduced-use patterns.}

\paragraph{Cholesky}  The Cholesky kernel iterates over the data in three regions,
first by performing a complex point operation, then reusing that several times
within a vector-scalar multiplication, and finally reusing vectors and scalars from
the previous two regions, while using a triangular memory access pattern.  The
unique aspect of Cholesky is that it requires not only several multi-reuse patterns,
but also that the length of the reuse dependences on the iteration -- it is inductive
on \texttt{k}.

\textbf{Feature 4: Supporting induction on the reuse pattern itself aids
parallelism of inductive access patterns.}

\begin{figure}[t]
\includegraphics[scale=0.483]{./figs/cholesky.pdf}
\caption{Computing kernels of Cholesky (\%'s: ideal exec. rate)}
\label{fig:chol-dep}
\end{figure}


\paragraph{Execution Rate}  Finally, notice also in Figures~\ref{fig:qr-dep} 
and~\ref{fig:chol-dep} that the execution rate is shown for each region.
This is calculated for an N=24 matrix,
assuming that all regions are being executed in parallel, and that
each inner loop is fully-pipelined (1-cycle per iteration),
this indicates the percentage of cycles which a region ``fires'' one computation. 

The implication of varying execution rate is 
that naively assigning \emph{proportional} execution resources to each static
computation will lead to hardware- under-utilization for low-rate regions.  One
approach for equalizing the execution rates is to vectorize the high-rate
loops. However, this can only be applied to a limited extent before vector overheads
prevail, and often the difference in firing rate is multiple integer factors.

An alternative solution to achieving acceptable hardware utilization is to
assign non-proportional execution resources to regions, based on their firing
rate.  What this translates to in terms of hardware, is that high-rate
instructions would be assigned fully-dedicated FU resources, while low-rate
instructions would be assigned a temporally
shared resource.  For example, in Cholesky, the
`inversion/sqrt' region can be assigned a shared resource for computation without
affecting the critical path of the application, since its firing rate is much lower.
This frees up more computational resources for the remaining instructions.
A similar situation exists in QR for the ``Divisor Calculation'' region.

\textbf{Feature 5: The hardware should enable a coexistence of high-rate regions
on dedicated hardware, and low-rate regions on shared hardware, while still
enabling communication between these regions.}

\begin{figure}[t]
\includegraphics[width=\linewidth]{figs/revel-cholesky.pdf}
\caption{Cholesky Mapped to Revel Abstractions}
\label{fig:rv-cholesky}
\end{figure}



==> cover.tex <==
\section*{Cover Letter: Exploiting Fine-Grain Ordered Parallelism in Dense Matrix
Algorithms (\#134)}

We genuinely thank the reviewers for their consideration, thoughtful suggestions, and
questions.  We first describe revisions, and then answer remaining questions.

\subsection*{Revisions based on Reviewer Suggestions}

\noindent \textbf{A1.} We added a thorough explanation of an example workload
with FGOP in the introduction (see Figure~\ref{fig:solver-fgop} in
Section~\ref{sec:intro}).  We also removed or explained the compiler terminology
(eg. vector-tiling).

\noindent \textbf{A2.} We added a characterization of the prevalence of FGOP
properties by studying linear algebra kernels from PolyBench, and the results
are in Table~\ref{tab:fgop-prev}. (\hyperlink{fgop-prev}{link}).

\noindent \textbf{A3.} We quantify challenges of exploiting FGOP for
traditional Vector/VonNeumann architectures through a case study of Cholesky in
Section~\ref{sec:challenges-existing}. 

\noindent \textbf{A4\&F1.} The potential of exploiting FGOP is best understood in the context of a
particular architecture, because it affects parallelism, data reuse, and
control overheads.  Therefore, we added an analysis to quantify incremental impact of exploiting 
each aspect of FGOP with hardware/software mechanisms in Figure~\ref{fig:inc}.  This required
writing five versions of each application to exploit each combination.
%Especially, when fine-grain dependence is enabled, most of the
%workloads we studies are accelerated considerably.

\noindent \textbf{C1.} Figure~\ref{fig:rv-cholesky} \texttt{local\_ld} parameters fixed.

\noindent \textbf{C2.} Though we think the intuitive definition of streams through loops
might be easier for some, we also added a formal stream definition in
Section~\ref{sec:exec-model} (\hyperlink{formalstream}{link}).

\noindent \textbf{D1.} We clarified the distinction between dedicated fabrics
(single-instruction per PE) and temporal fabrics (multiple-instructions per PE)
in Section~\ref{sec:het-fab}, as well as why its important for all dataflows to
be executed on a fabric that supports data-triggered execution.  

\noindent \textbf{F2.} We expand on the modeling of REVEL in
Section~\ref{sec:methodology} by detailing all hardware blocks and params
in Table~\ref{tab:arch-param} and clarifying that all blocks are modeled at a
cycle level within gem5.  We do not believe there are any significant optimistic
assumptions.  Also, we clarified that all blocks for one REVEL
lane are synthesized for power/area estimates \hyperlink{allblocks}{(link)}.  

\noindent \textbf{Commitment to Open Source} We are confident our simulator is
accurate, and we feel the infrastructure can have value to
the community.  Therefore we will release \emph{all} simulator, compiler, and
applications through permissive open source license on acceptance, for the
community to inspect and build upon (footnote in Sec~\ref{sec:methodology}).

\subsection*{Response to Reviewer Questions/Comments}

\paragraph{A1. What is ordered dependency (as opposed to unordered)?}  
We clarify in Section~\ref{sec:fgop} that we are referring to \emph{ordered} 
with respect to the corresponding static instructions; an ordered dependence
between statements s1 and s2 means that s1 produces values in the order that s2 consumes them.
Eg. if s2 consumes values from s1 in backwards order, this is unordered.

\paragraph{A2. What is an iteration domain?} See Section~\ref{sec:exec-model}.

\paragraph{A3. What is a stream?}  A pattern of memory accesses or data movements.  Formal def. in 
Section~\ref{sec:exec-model}.

\paragraph{A4. What is ``reuse'' in a dependence?} When a consuming instruction
 uses the same value from a producing instr. multiple times (often a loop invariant).

\paragraph{A5. Why these workloads?} Because they are important for (and representative of) 
signal processing, which forms a coherent domain around which a programmable engine can target.
Briefly discussed in Sec~\ref{sec:background}.

\paragraph{A6. Why does REVEL support FGOP and traditional parallelism?}  Because 1. workloads in
this domain are diverse and several require traditional parallelism, 2. some traditional parallelism
is available even in FGOP-centric workloads, and 3. traditional parallelism is easy and profitable
to exploit in hardware.
 
\paragraph{B1. Do ASICs exploit FGOP too?}
Yes, our optimistic ASIC models assume perfect exploitation of FGOP, using the same algorithm as REVEL.


\paragraph{B2. How does this compare to loop parallelization through reuse distance?}  As far as we understand,
we target a different class of workloads: traditional exploitation of loop-dependence distance relies 
on fixed-distance dependences, whereas we can exploit inductive change in reuse distance.

\paragraph{C1. Paper does not explain the dataflow compiler; How are the independent computations mapped to the compute fabric?} 
Though the compiler is not the focus or contribution, Section~\ref{sec:compiler} explains that we implemented a simulated annealing approach to map independent dataflow graphs to compute fabric.

\paragraph{C2. How can the outer k loop of Cholesky be paralleled when there is a
dependence across it?} Iterations of k are mapped to adjacent lanes.  We
support dependences between lanes in the execution model with fine-grain
ordered dependences, in the ISA with \texttt{XFER} commands, and in the
microarchitecture with the \texttt{XFER} unit (and corresponding buses).

\paragraph{C3. In Figure~\ref{fig:solver-dfg}, shouldn't (n-j:1) be (j:1)?} We are confident it is (n-j:1).

\paragraph{C4. In Figure~\ref{fig:solver-streams}, the '/' op. has no 'i' loop. So what does $C_i$ mean here?} \hyperlink{inneriter}{See added footnote}.

\paragraph{D1. Unimpressive Power/Area over ASIC -- hard to convince chip manufactures to use REVEL}  
Area and power overheads are \emph{extremely} optimistic for ASIC, and include NO control or 
buffering overhead (just SRAMs and FUs).  Being lower area than the combined highly-ideal ASIC is still
promising.

\paragraph{F1. Compare to Plasticine/Swarm}  With more space we can do a more rigorous
comparison to their abstractions, beyond broad statements in related work.

\paragraph{F2. Why can REVEL outperform DSPs by order-of-magnitude even though
they were designed to target these workloads?}  FGOP is the dominant form of parallelism,
which is difficult to express/exploit in a single-threaded VonNeumann model (regions get serialized),
or with threads (synchronization dominates).  VonNeumann+threading have become such mainstays in hardware/software
 that it is difficult to overcome inertia.  

\newpage



==> overview.tex <==
\section{Overview} \label{sec:overview}

In this section, we present an overview of REVEL's execution model by
motivating the domain and its challenges, explain the design setting and
requirements, and outlining our solution, including the relevant background.

\subsection{Accelerator Setting and Requirements}

\paragraph{Accelerator Setting}  We consider here a hardware setting where any
sensors and accelerators both have high-bandwidth access to on-chip SRAM.
 This hardware organization is applicable to mobile processors and
5G wireless base-stations.  

\paragraph{Requirements} In this setting, mainstream approaches
were traditionally  VLIW-based multi-core DSPs, but this has shifted
towards ASICs.  Any programmable replacement for a set of ASICs must be:

\begin{itemize}
\item \textbf{Performance Equivalent:}  The performance 
should meet the throughput capabilities of existing ASICs.
\item \textbf{Power/Area Neutral:}  
Have ideally less than 2$\times$ power overheads, and be the same or less
area.
\item \textbf{Conceivably General}:  
Should be conceivably generalizable to a variety of DSP algorithms.
\item \textbf{Flexible Metric:}  Be able to provide not only high throughput, 
but also low latency.
\end{itemize}

\subsection{Workload Kernels}
The specification for 5G wireless is in the early stages
of being completed~\cite{draft5g}, and will require higher
throughput, lower latency, and lower power signal processing 
capabilities.  However, rather than focus on meeting
specific end-to-end targets, we find it more insightful to 
instead drive our approach by attempting to
achieve near-ASIC levels of performance and power in scalable fashion.

Below we highlight the digital signal processing kernels that serve as our targets,
and put them in three categories based on their architecture-related characteristics.

\begin{figure}
\begin{center}
\includegraphics[width=0.99\linewidth]{figs/background.pdf}
\end{center}
\captionof{figure}{Background: Stream-Dataflow ISA and Hardware Impl.}
\label{fig:background}
\end{figure}


\paragraph{Regular Matrix Operations}  
There are a number of well-understood regular kernels,
like matrix-matrix and matrix-vector multiplication, which are quite important in
DSP algorithms.  These also include filters (eg. \emph{polyphasic}~\cite{polyphase},  
\emph{Centro-symmetric kernels}~\cite{centro-symm}, and \emph{half-band filters}~\cite{half-band}).  Also, these include FFT algorithms for transforming between time
and frequency representations of signals.
These workloads have control patterns which lend themselves nicely to vector machines,
but are still difficult to parallelize across cores when the matrix size is small.

\paragraph{Matrix Factorization/Decomposition}  Matrix factorization and matrix
decomposition are critical DSP algorithms which are much more challenging to
improve.  These include \emph{Singular Value Decomposition},
used for noise reduction~\cite{speech-svd},  \emph{QR
Decomposition}, used for signal detection for multiple-input multiple output
(MIMO)~\cite{qr-dsp}, and \emph{Cholesky decomposition} used in channel
estimation and equalization~\cite{cholesky-dsp,lmmse-wcdma}. 

While these workloads are still dense linear
algebra, they are non-trivial for vector processors.  Because these algorithms
are induction based, the size of the intermediate vectors which they operate
over change.  This leads to two problems: 1. control: the lengths of vectors
much be updated at each step; and 2. indivisibility: vector data for each row
of computation is typically not divisible by the vector size.  Both of the
above add instruction overhead.

Furthermore, it is often the case that the sub-computations of the matrix can be
performed in parallel.  For example, parallelization of the outer
loop in Cholesky Decomposition.
%, by observing the dependeces
%in a more fine-grain way, it is easy to find that next iteration's computation
%can start when the current iteration produces the values in the first row.
However, because there are some dependences between these
coarse-grain phases, VonNeumann-based vector machines have difficulty executing
these in parallel as it would introduce multi-threading overhead; however, this
is trivially simple for an ASIC, which can have specialized synchronization for
the simple fine-grain dependence patterns.

\paragraph{Cross-Cutting Concerns}  One key aspect of the workload setting is
that there are many matrices to be processed in parallel, but they are of
relatively small sizes.  For example, due to the number of inputs/outputs in
MIMO communication, dimension 12-32 matrices are common for QR decomposition.
While small matrices are cache friendly, they greatly exacerbate control overhead.

\emph{Summary: The major challenges for DSP workloads are in hiding
control overhead and enabling parallelism while supporting fine-grain dependences.}

\subsection{Insights and Accelerator Baseline}
The limited benefits of vectorization means that it is necessary to exploit
vector parallelism in concert 
with coarse grain pipelining within and across fine-grain dependent code regions.
We suggest that the spatial architecture paradigm is a good starting
point; a spatial architecture exposes its execution, communication, and
data-reuse resources to the ISA.  These architectures are promising because they
generally support deep pipelining of computation graphs with low hardware overhead, as
well as various forms of operand communication.  

However, the aforementioned challenges of supporting inductive control and
parallelism with fine-grain dependences remain for spatial architectures.  
One way to address the problem is to embed general control flow support 
at each computation unit (eg. Triggered
Instructions~\cite{triggered-insts}, TRIPS~\cite{trips}, or 
WaveScalar~\cite{wavescalar}), but these impose a significant power and
area overhead of an ASIC.   On the other end of the spectrum, there are
those that impose a strict static-dataflow model of execution (eg.
a systolic array~\cite{systolicarrays,systolicarrays2} or other reconfigurable
array like FPCA~\cite{fpca} or Morphosys~\cite{morphosys}), but these are
not amenable to the access or dependence patterns.

% RSVP~\cite{rsvp}  (e.g. Softbrain~\cite{stream-dataflow},  DRISSA~\cite{drissa}, or DPU~\cite{venkat-dpu}), (e.g. Plasticine~\cite{plasticine}, Charm~\cite{charm}, Camel~\cite{camel}, ).

Our goal is to be able to get the best of both worlds, achieving performance 
of the desired control and parallelism paradigm with close-to-ASIC power and
area overheads.  Our insight is simply that both are achievable if these inductive
control and communication primitives are available in the hardware/software 
interface.  In order to perform this specialization easily, we start with 
architecture and execution model that has been proven to be amenable to extremely low-overhead hardware, specifically  stream-dataflow~\cite{stream-dataflow}. 

\paragraph{Stream-dataflow Background}
An example stream-dataflow program is in Figure~\ref{fig:background}(b).
The defining feature of a stream-based ISA is the ability to express 
variable-length access patterns.  For example,
\texttt{load a[i*k]} where k is 
constant and i increases from 0 to n.  
The execution model also uses decoupled access-execute~\cite{dae},
to separate memory streams from a dataflow graph 
representing repeated computations.
A first-in first-out (FIFO) queue interfaces the
computation units and high-bandwidth local memories.

\begin{figure}
\vspace{-0.12in}	
\begin{center}
\includegraphics[width=\linewidth]{figs/revel-model.pdf}
\end{center}
\caption{REVEL Program and Execution Model Example}
\label{fig:revel-model}
\end{figure}

An implementation, Softbrain~\cite{stream-dataflow}, is shown in
Figure~\ref{fig:background}(a).
This design combines a coarse-grain reconfigurable array for 
dataflow graph execution, with a set of streaming-memory engines
to process streams specified in the program.  
A control core sends stream-commands and coordinates the execution.
We compare against this design in our evaluation.


\subsection{Proposed Architecture/Execution Model: REVEL}

Our work proposes the REVEL architecture, 
which is a novel execution model that combines
vectorized-control with a streaming model of computation which builds
off of stream-dataflow.  A REVEL program is composed of a vector-stream
program and some number of dataflow graphs representing the computation.
The vector-stream code is a coarse grain, partially ordered
 specification of memory access, data communication and
reuse patterns flowing into and out-of dataflow graphs.   Vectorization allows a
single control stream to be broadcast to many dataflow graphs.


A high-level version of a REVEL program is shown in
Figure~\ref{fig:revel-model}, which is a simple square-root and accumulate
kernel.  The REVEL program can parallelize the outer $j$, loop, essentially
creating multiple independent dataflow graphs (DFGs).  The streaming reuse of
the square-root is expressed as a coarse grain stream, which enables decoupled
parallelism of square-root's $j+1$ iteration with inner loops $j$ iteration.
Advanced features are explained with an example in
Section~\ref{sec:revel}.

%In terms of the hardware, REVEL introduces an inductive address generator
%to handle changing vector lenghts, 


%For simplicity, we also refer to the architecture implementation as REVEL,
%which is shown in Figure~\ref{fig:revel-overview} (page~\pageref{fig:revel-overview}).
%We describe detailed hardware the innovations below.

%\paragraph{Control Specialization} 
%\begin{itemize}
%\item \textbf{Software: Inductive Control}  
%\item \textbf{Hardware: Inductive Address Generator}
%\item \textbf{Hardware: Configurable Reuse}
%\end{itemize}
%
%\paragraph{Parallelism Specialization} 
%\begin{itemize}
%\item \textbf{Software: Inter-DFG Communication} 
%\item \textbf{Hardware: Multi-DFG/CGRA Support}
%\item \textbf{Hardware: Temporal Mapping Regions}
%\end{itemize}



==> todo.tex <==
Not Done:
* Improve area/power model
* Figure for abstractions and updating writing? (I might need to help writing?)
* Make everything Consistent!
  * Make all writing and analysis consistent with results graphs and figures
  * make all summary numbers consisdent
  * make sure we use the same terminology for everything consistently
* Minor things you should do if you have time:
  * Check if you agree with analysis of FGOP
  * Check if you agree with analysis of adding FGOP to other accelerators
  * Make ASIC analytical Models parameterized by various latencies (eg. div lat)
  * add citation for number of antennas?
  * add "matrix width" label on Figure 8 and Figure 1 for the x-axis (without increasing figure size too much)
* Final spellcheck
* Final grammarcheck
* Update abstract on hotcrp
* Add old reviews on hotcrp (DO NOT UNDER ANY CIRCUMSTANCES INCLUDE ANY OF OUR EMAILS OR OTHER IDENTIFYING INFORMATION)
* Make version highlighted with changes (just use adobe or PDF editor to add comments) -- I might be able to do if time

Done:
* remove multi-reuse terminology
* Add discussion about applying REVEL principles to Plasticine/DySER (i did OOO core instead)
* Add prevalence discussion
* Make all results complete
* Improve text size on Figure 7: prevlanece of FGOP properties
* Minor things you should do if you have time:
  * Check if you agree with analysis of FGOP
  * Check if you agree with analysis of adding FGOP to other accelerators
  * add citation for number of antennas?
  * add "matrix width" label on Figure 8 and Figure 1 for the x-axis (without increasing figure size too much)

